Programming Strategies for Irregular Algorithms on the Emu Chick

The Emu Chick prototype implements migratory memory-side processing in a novel hardware system. Rather than transferring large amounts of data across the system interconnect, the Emu Chick moves lightweight thread contexts to near-memory cores before the beginning of each remote memory read. Previous work has characterized the performance of the Chick prototype in terms of memory bandwidth and programming differences from more typical, non-migratory platforms, but there has not yet been an analysis of algorithms on this system. This work evaluates irregular algorithms that could benefit from the lightweight, memory-side processing of the Chick and demonstrates techniques and optimization strategies for achieving performance in sparse matrix-vector multiply operation (SpMV), breadth-first search (BFS), and graph alignment across up to eight distributed nodes encompassing 64 nodelets in the Chick system. We also define and justify relative metrics to compare prototype FPGA-based hardware with established ASIC architectures. The Chick currently supports up to 68x scaling for graph alignment, 80 MTEPS for BFS on balanced graphs, and 50\% of measured STREAM bandwidth for SpMV.

==> style/comments.tex <==
%%% Macros to allow authors to make comments in-line in the text
%%% Modified by Jeff Young, 12/14/17
%%% To use: \jsy{This is a comment that should show up in-line in the text}

%Comment for Eric
\newcommand{\rem}[1]{\marginpar{\textcolor{red}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{red}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}

\newcommand{\remname}[2]{{\marginpar{\textcolor{red}{$\star$ #2}}\sf{\normalsize{\textcolor{red}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\eh}[1]{\remname{#1}{eh}}

%Comment for Jason
\newcommand{\remjr}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamejr}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\jr}[1]{\remnamejr{#1}{jr}}

%Comment for Jeff
\newcommand{\remjy}[1]{\marginpar{\textcolor{orange}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{orange}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamejy}[2]{{\marginpar{\textcolor{orange}{$\star$ #2}}\sf{\normalsize{\textcolor{orange}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\jsy}[1]{\remnamejy{#1}{jsy}}

%Comment for Srinivas
\newcommand{\remse}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamese}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\se}[1]{\remnamese{#1}{se}}

%Comment for Jiajia
\newcommand{\remjli}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamejli}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\jli}[1]{\remnamejli{#1}{jli}}

%Comment for Srinivas
\newcommand{\rempl}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamepl}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\pl}[1]{\remnamepl{#1}{pl}}




==> style/pkgs.tex <==
%% Separate file for definitions and packages
%% Many of the contributions are from Dr. Rich Vuduc or his group. 

%Include Rich's packages and standard typography
\usepackage{style/my-stdpkgs}
\usepackage{style/my-typography}
\usepackage{acronym}
\usepackage{microtype} % Space-squishing via kerning
\usepackage{afterpage}

%From Piyush's SuperLU paper
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
%Use this or Latin input encoding
%\usepackage[utf8]{inputenc}
\usepackage{verbatim}
\usepackage{textcomp}

\setcounter{secnumdepth}{3}

\usepackage{array,ragged2e}

%\usepackage{graphicx}
%\usepackage{amsmath}
\usepackage{float}
\usepackage{amsfonts}
%\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{morefloats}

%%Used for SuperLU listings
%\newenvironment{lyxcode}
%{\par\begin{list}{}{
%\setlength{\rightmargin}{\leftmargin}
%\setlength{\listparindent}{0pt}% needed for AMS classes
%\raggedright
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\normalfont\ttfamily}%
 %\item[]}
%{\end{list}}
%\theoremstyle{plain}
%\newtheorem{thm}{\protect\theoremname}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.


%% Fix for paragraph formatting that is non-bolded with IEEEtran
\makeatletter
\def\@IEEEsectpunct{.\ \,}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
{0ex}{\normalfont\normalsize\sffamily\bfseries}}
\makeatother

\usepackage{algorithm}
\usepackage[noend]{algorithmic}

%Define the following variables used in equations - s, min_parallelism, min_threshold,
%max_threshold,
\newcommand{\vrtxs}{\textit{s}\xspace}
\newcommand{\minpar}{\textsc{min\_parallelism}\xspace}
\newcommand{\minthrsh}{\textsc{min\_threshold}\xspace}
\newcommand{\maxthrsh}{\textsc{max\_threshold}\xspace}

%\newcommand{\TODO}[1]{{\color{red}TODO: #1}}
\newcommand{\TOCITE}{\TODO{CITE}}

% === Document/project-specific macros ===
%
\acrodef{PCIe}{Peripheral Component Interface Express}
\newcommand{\PCIe}{\ac{PCIe}\xspace}

% Common libraries and frameworks

\newcommand{\MPI}{{\scshape mpi}\xspace}
\newcommand{\OpenMP}{{\scshape openmp}\xspace}

%% Algorithms
%\acrodef{SVD}[SVD]{singular value decomposition}
%\newcommand{\SVD}{\ac{SVD}\xspace}
%
%% Some sparse matrix formats
%\acrodef{CSH}[CSH]{compressed sparse hyperplane}
%\newcommand{\CSH}{\ac{CSH}\xspace}
%\acrodef{COO}[COO]{coordinate}
%\newcommand{\COO}{\ac{COO}\xspace}


% === END document/project-specific macros ===


==> style/symbols.tex <==
\acrodef{DVFS}[DVFS]{dynamic frequency and voltage scaling}
\newcommand{\DVFS}{\ac{DVFS}\xspace}

\acrodef{DFS}[DFS]{dynamic frequency scaling}
\newcommand{\DFS}{\ac{DFS}\xspace}

\acrodef{SSSP}[SSSP]{single-source shortest path}
\newcommand{\SSSP}{\ac{SSSP}\xspace}

\acrodef{GPU}[GPU]{graphics co-processors}
\newcommand{\GPU}{\ac{GPU}\xspace}


\newcommand{\roadNet}{\textsf{Cal}\xspace}
\newcommand{\sfNet}{\textsf{wikipedia-20051105}\xspace}
\newcommand{\sfNetShort}{\textsf{Wikipedia}\xspace}

\newcommand{\advanceS}{\textsf{advance}\xspace}
\newcommand{\filterS}{\textsf{filter}\xspace}
\newcommand{\bisectFrontierS}{\textsf{bisect-frontier}\xspace}
\newcommand{\bisectFarQueueS}{\textsf{bisect-far-queue}\xspace}

\newcommand{\advanceX}[1]{\ensuremath{X^{(1)}_{#1}}\xspace}
\newcommand{\filterX}[1]{\ensuremath{X^{(2)}_{#1}}\xspace}
\newcommand{\bisectFrontierX}[1]{\ensuremath{X^{(3)}_{#1}}\xspace}
\newcommand{\bisectFarQueueX}[1]{\ensuremath{X^{(4)}_{#1}}\xspace}

\newcommand{\dynDelta}[1]{\ensuremath{\delta_{#1}}\xspace}
\newcommand{\changeDelta}[1]{\ensuremath{\Delta \dynDelta{#1}}}
\newcommand{\advanceE}{\textsf{\textsc{Advance-Model}}\xspace}
\newcommand{\bisectE}{\textsf{\textsc{Bisect-Model}}\xspace}
\newcommand{\rebalancerS}{\textsf{rebalancer}\xspace}

\newcommand{\advanceXest}[1]{\ensuremath{\hat{X}^{(1)}_{#1}}\xspace}
\newcommand{\filterXest}[1]{\ensuremath{\hat{X}^{(2)}_{#1}}\xspace}

\newcommand{\variant}[1]{\overline{#1}}

\newcommand{\boundary}[1]{\ensuremath{B_{#1}}\xspace}
\newcommand{\MAXINT}{\ensuremath{\mathtt{MAX\_INT}}\xspace}

